CeMon: A Cost-effective Flow Monitoring System in Software Defined Networks

Network monitoring and measurement are crucial in network management to facilitate quality of service routing and performance evaluation. Software Defined Networking (SDN) makes network management easier by separating the control plane and data plane. Network monitoring in SDN is relatively light-weight since operators only need to install a monitoring module into the controller. Active monitoring techniques usually introduce extra overhead into the network. The state-of-the-art approaches utilize sampling, aggregation and passive measurement techniques to reduce measurement overhead. However, little work has focused on reducing the communication cost of network monitoring. Moreover, most of the existing approaches select polling switch nodes by sub-optimal local heuristics.Inspired by the visibility and central control of SDN, we propose CeMon, a generic low-cost high-accuracy monitoring system that supports various network management tasks. We first propose a Maximum Coverage Polling Scheme (MCPS) to optimize the polling cost for all active flows. The problem is formulated as a weighted set cover problem which is proved to be NP-hard. Heuristics are presented to obtain the polling scheme efficiently and handle traffic dynamics practically. In order to balance the cost and flexibility, an Adaptive Fine-grained Polling Scheme (AFPS) is proposed as a complementary method to implement flow level measurement tasks. Three sampling algorithms are further proposed to eliminate measurement overhead while maintain high accuracy. Both emulation and simulation results show that MCPS reduces more than 50% of the communication cost with negligible loss of accuracy for different topologies and traffics. We also use real traces to demonstrate that AFPS reduces the cost by up to 20% with only 1.5% loss in accuracy.

==> bio.tex <==
\parpic{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Zhiyang}}
\noindent {\bf Zhiyang Su} received the B.E. degree in computer science and technology from the China University of Geosciences (Beijing) in 2009, and the M.S. degree in computer network and application from the Peking University in 2012. Currently, he is pursuing Ph.D. degree in the Hong Kong University of Science and Technology. His research interests include software defined networks and data center networks.

\parpic{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Ting}}
\noindent {\bf Ting Wang} received his B.S. degree from the University of Science and Technology Beijing, China, in 2008, and received his M.E. degree from the Warsaw University of Technology, Poland, in 2011. From 02.2012 to 08.2012 he interned as a research assistant in the Institute of Computing Technology, Chinese Academy of Sciences. He is currently working towards the Ph.D. degree in computer science and engineering in the Hong Kong University of Science and Technology. His research interests include data center networks, cloud computing, green computing, and software defined network.

\parpic{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Yu}}
\noindent {\bf Yu Xia} is currently a postdoctoral fellow in Department of Computer Science and Engineering, the Hong Kong University of Science and Technology. He received the Ph.D. in computer science from the Southwest Jiaotong University, China. He was a joint Ph.D student and a visiting scholar at Polytechnic Institute of New York University. His research interests include high-performance packet switches, data center networks and network architectures.

\parpic{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/Hamdi}}
\noindent {\bf Mounir Hamdi} received the B.S. degree in Electrical Engineering - Computer Engineering minor (with distinction) from the University of Louisiana in 1985, and the M.S. and the Ph.D. degrees in Electrical Engineering from the University of Pittsburgh in 1987 and 1991, respectively. He is a Chair Professor at the Hong Kong University of Science and Technology. He is an IEEE Fellow for contributions to design and analysis of high-speed packet switching.

